Albert, an intermediate smart-contract language for the Tezos blockchain

Tezos is a smart-contract blockchain. Tezos smart contracts are written in a low-level stack-based language called Michelson. In this article we present Albert, an intermediate language for Tezos smart contracts which abstracts Michelson stacks as linearly typed records. We also describe its compiler to Michelson, written in Coq, that targets Mi-Cho-Coq, a formal specification of Michelson implemented in Coq.

==> toplevel_definition.tex <==
% generated by Ott 0.29 from: latex.ott toplevel_definition.ott
\newcommand{\toplevel_definitiondrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\toplevel_definitiondrulename{#4}}}
\newcommand{\toplevel_definitionusedrule}[1]{\[#1\]}
\newcommand{\toplevel_definitionpremise}[1]{ #1 \\}
\newenvironment{toplevel_definitiondefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{toplevel_definitionfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\toplevel_definitionfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\toplevel_definitionnt}[1]{\mathit{#1}}
\newcommand{\toplevel_definitionmv}[1]{\mathit{#1}}
\newcommand{\toplevel_definitionkw}[1]{\mathbf{#1}}
\newcommand{\toplevel_definitionsym}[1]{#1}
\newcommand{\toplevel_definitioncom}[1]{\text{#1}}
\newcommand{\toplevel_definitiondrulename}[1]{\textsc{#1}}
\newcommand{\toplevel_definitioncomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\toplevel_definitioncompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\toplevel_definitioncomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\toplevel_definitiongrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\toplevel_definitionmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\toplevel_definitionrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\toplevel_definitionprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\toplevel_definitionfirstprodline}[6]{\toplevel_definitionprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\toplevel_definitionlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\toplevel_definitionfirstlongprodline}[2]{\toplevel_definitionlongprodline{#1}{#2}}
\newcommand{\toplevel_definitionbindspecprodline}[6]{\toplevel_definitionprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\toplevel_definitionprodnewline}{\\}
\newcommand{\toplevel_definitioninterrule}{\\[5.0mm]}
\newcommand{\toplevel_definitionafterlastrule}{\\}
\renewcommand{\toplevel_definitionkw}{\texttt}

\newcommand{\toplevel_definitionmetavars}{
\toplevel_definitionmetavartabular{

}}

\newcommand{\toplevel_definitiontvar}{
\toplevel_definitionrulehead{\toplevel_definitionnt{tvar}}{::=}{}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionkw{id}} {\textsf{S}}{}{}{}}

\newcommand{\toplevel_definitionfvar}{
\toplevel_definitionrulehead{\toplevel_definitionnt{fvar}}{::=}{}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionkw{id}} {\textsf{S}}{}{}{}}

\newcommand{\toplevel_definitionty}{
\toplevel_definitionrulehead{\toplevel_definitionnt{ty}  ,\ \toplevel_definitionnt{a}  ,\ \toplevel_definitionnt{b}  ,\ \toplevel_definitionnt{c}}{::=}{\toplevel_definitioncom{Type}}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionnt{tvar}}{}{}{}{\toplevel_definitioncom{Type variable}}}

\newcommand{\toplevel_definitionf}{
\toplevel_definitionrulehead{\toplevel_definitionnt{f}}{::=}{\toplevel_definitioncom{Function symbol}}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionnt{fvar}}{}{}{}{}}

\newcommand{\toplevel_definitiondefinition}{
\toplevel_definitionrulehead{\toplevel_definitionnt{definition}}{::=}{\toplevel_definitioncom{Toplevel definition}}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionkw{type} \, \toplevel_definitionnt{tvar}  \texttt{=}  \toplevel_definitionnt{ty}}{}{}{}{}\toplevel_definitionprodnewline
\toplevel_definitionprodline{|}{\toplevel_definitionkw{def} \, \toplevel_definitionnt{fvar}  ~\texttt{:}~  \toplevel_definitionnt{ty}  ~\texttt{->}~  \toplevel_definitionnt{ty'}  \texttt{=} \, \toplevel_definitionkw{instruction}}{}{}{}{}}

\newcommand{\toplevel_definitionprog}{
\toplevel_definitionrulehead{\toplevel_definitionnt{prog}}{::=}{\toplevel_definitioncom{Toplevel definition}}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\toplevel_definitionnt{definition}}{}{}{}{}\toplevel_definitionprodnewline
\toplevel_definitionprodline{|}{\toplevel_definitionnt{definition} \, \toplevel_definitionnt{prog}}{}{}{}{}}

\newcommand{\toplevel_definitiong}{
\toplevel_definitionrulehead{\Gamma}{::=}{\toplevel_definitioncom{Typing context (for inlined definitions)}}\toplevel_definitionprodnewline
\toplevel_definitionfirstprodline{|}{\Gamma  \toplevel_definitionsym{,}  \toplevel_definitionnt{fvar}  ~\texttt{:}~  \toplevel_definitionnt{ty}  \Rightarrow  \toplevel_definitionnt{ty'}}{}{}{}{}\toplevel_definitionprodnewline
\toplevel_definitionprodline{|}{\Gamma  \toplevel_definitionsym{,}  \toplevel_definitionnt{tvar}  \texttt{=}  \toplevel_definitionnt{ty}}{}{}{}{}}

\newcommand{\toplevel_definitiongrammar}{\toplevel_definitiongrammartabular{
\toplevel_definitiontvar\toplevel_definitioninterrule
\toplevel_definitionfvar\toplevel_definitioninterrule
\toplevel_definitionty\toplevel_definitioninterrule
\toplevel_definitionf\toplevel_definitioninterrule
\toplevel_definitiondefinition\toplevel_definitioninterrule
\toplevel_definitionprog\toplevel_definitioninterrule
\toplevel_definitiong\toplevel_definitionafterlastrule
}}

% defnss
% defns Jtype
%% defn fresh_tvar

\newcommand{\toplevel_definitiondefntypingXXfreshXXtvar}[1]{\begin{toplevel_definitiondefnblock}[#1]{$ \toplevel_definitionnt{tvar}  \notin \mathsf{FV}( \toplevel_definitionnt{ty} ) $}{\toplevel_definitioncom{Type variable freshness}}
\end{toplevel_definitiondefnblock}}


\newcommand{\toplevel_definitiondefnsJtype}{
\toplevel_definitiondefntypingXXfreshXXtvar{}}

\newcommand{\toplevel_definitiondefnss}{
\toplevel_definitiondefnsJtype
}

\newcommand{\toplevel_definitionall}{\toplevel_definitionmetavars\\[0pt]
\toplevel_definitiongrammar\\[5.0mm]
\toplevel_definitiondefnss}



==> variant.tex <==
% generated by Ott 0.29 from: latex.ott pattern_matching.ott variant.ott
\newcommand{\variantdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\variantdrulename{#4}}}
\newcommand{\variantusedrule}[1]{\[#1\]}
\newcommand{\variantpremise}[1]{ #1 \\}
\newenvironment{variantdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{variantfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\variantfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\variantnt}[1]{\mathit{#1}}
\newcommand{\variantmv}[1]{\mathit{#1}}
\newcommand{\variantkw}[1]{\mathbf{#1}}
\newcommand{\variantsym}[1]{#1}
\newcommand{\variantcom}[1]{\text{#1}}
\newcommand{\variantdrulename}[1]{\textsc{#1}}
\newcommand{\variantcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\variantcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\variantcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\variantgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\variantmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\variantrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\variantprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\variantfirstprodline}[6]{\variantprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\variantlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\variantfirstlongprodline}[2]{\variantlongprodline{#1}{#2}}
\newcommand{\variantbindspecprodline}[6]{\variantprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\variantprodnewline}{\\}
\newcommand{\variantinterrule}{\\[5.0mm]}
\newcommand{\variantafterlastrule}{\\}
\renewcommand{\variantkw}{\texttt}

\newcommand{\variantmetavars}{
\variantmetavartabular{
 $ \variantmv{k} $ &  \\
}}

\newcommand{\variantbranchesXXrhs}{
\variantrulehead{\variantnt{branches\_rhs}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantnt{pattern_{{\mathrm{1}}}}  ~\texttt{->}~  \variantnt{rhs_{{\mathrm{1}}}}  ~\texttt{|}~ \, ... \, ~\texttt{|}~  \variantnt{pattern_{\variantmv{k}}}  ~\texttt{->}~  \variantnt{rhs_{\variantmv{k}}}}{}{}{}{}}

\newcommand{\variantrhs}{
\variantrulehead{\variantnt{rhs}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantkw{match} \, \variantnt{var} \, \variantkw{with} \, \variantnt{branches\_rhs} \, \variantkw{end}}{}{}{}{}}

\newcommand{\variantbranchesXXins}{
\variantrulehead{\variantnt{branches\_ins}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantnt{pattern_{{\mathrm{1}}}}  ~\texttt{->}~  \variantnt{ins_{{\mathrm{1}}}}  ~\texttt{|}~ \, ... \, ~\texttt{|}~  \variantnt{pattern_{\variantmv{k}}}  ~\texttt{->}~  \variantnt{ins_{\variantmv{k}}}}{}{}{}{}}

\newcommand{\variantinstruction}{
\variantrulehead{\variantnt{instruction}  ,\ \variantnt{ins}  ,\ \variantnt{I}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantkw{match} \, \variantnt{var} \, \variantkw{with} \, \variantnt{branches\_ins} \, \variantkw{end}}{}{}{}{}}

\newcommand{\variantconstructor}{
\variantrulehead{\variantnt{constructor}  ,\ \variantnt{C}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantkw{id}} {\textsf{S}}{}{}{}}

\newcommand{\variantlabel}{
\variantrulehead{\variantnt{label}  ,\ \variantnt{l}  ,\ \variantnt{var}  ,\ \variantnt{x}}{::=}{\variantcom{Label / variable}}}

\newcommand{\variantty}{
\variantrulehead{\variantnt{ty}  ,\ \variantnt{a}  ,\ \variantnt{b}  ,\ \variantnt{c}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantnt{vty}}{}{}{}{}}

\newcommand{\variantvty}{
\variantrulehead{\variantnt{vty}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\texttt{[}  \variantnt{constructor_{{\mathrm{1}}}}  ~\texttt{:}~  \variantnt{ty_{{\mathrm{1}}}}  ~\texttt{|}~ \, ... \, ~\texttt{|}~  \variantnt{constructor_{\variantmv{k}}}  ~\texttt{:}~  \variantnt{ty_{\variantmv{k}}}  \texttt{]}}{}{}{}{}}

\newcommand{\variantf}{
\variantrulehead{\variantnt{f}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\texttt{(}  \variantnt{constructor}  ~\texttt{:}~  \variantnt{vty}  \texttt{)}}{}{}{}{}}

\newcommand{\variantpattern}{
\variantrulehead{\variantnt{pattern}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\variantkw{\_}}{}{}{}{}\variantprodnewline
\variantprodline{|}{\variantnt{constructor} \, \variantnt{var}}{}{}{}{}}

\newcommand{\variantvalue}{
\variantrulehead{\variantnt{value}  ,\ \variantnt{val}}{::=}{}\variantprodnewline
\variantfirstprodline{|}{\texttt{(}  \variantnt{constructor} \, \variantnt{value}  ~\texttt{:}~  \variantnt{vty}  \texttt{)}}{}{}{}{}}

\newcommand{\variantgrammar}{\variantgrammartabular{
\variantbranchesXXrhs\variantinterrule
\variantrhs\variantinterrule
\variantbranchesXXins\variantinterrule
\variantinstruction\variantinterrule
\variantconstructor\variantinterrule
\variantlabel\variantinterrule
\variantty\variantinterrule
\variantvty\variantinterrule
\variantf\variantinterrule
\variantpattern\variantinterrule
\variantvalue\variantafterlastrule
}}

% defnss
% defns Jtype
%% defn fresh_tvar

\newcommand{\variantdefntypingXXfreshXXtvar}[1]{\begin{variantdefnblock}[#1]{$ \variantkw{tvar}  \notin \mathsf{FV}( \variantnt{ty} ) $}{\variantcom{Type variable freshness}}
\end{variantdefnblock}}


\newcommand{\variantdefnsJtype}{
\variantdefntypingXXfreshXXtvar{}}

\newcommand{\variantdefnss}{
\variantdefnsJtype
}

\newcommand{\variantall}{\variantmetavars\\[0pt]
\variantgrammar\\[5.0mm]
\variantdefnss}


